TBD: Benchmarking and Analyzing Deep Neural Network Training

The recent popularity of deep neural networks (DNNs) has generated a lot of research interest in performing DNN-related computation efficiently. However, the primary focus is usually very narrow and limited to (i) inference -- i.e. how to efficiently execute already trained models and (ii) image classification networks as the primary benchmark for evaluation. Our primary goal in this work is to break this myopic view by (i) proposing a new benchmark for DNN training, called TBD (TBD is short for Training Benchmark for DNNs), that uses a representative set of DNN models that cover a wide range of machine learning applications: image classification, machine translation, speech recognition, object detection, adversarial networks, reinforcement learning, and (ii) by performing an extensive performance analysis of training these different applications on three major deep learning frameworks (TensorFlow, MXNet, CNTK) across different hardware configurations (single-GPU, multi-GPU, and multi-machine). TBD currently covers six major application domains and eight different state-of-the-art models. We present a new toolchain for performance analysis for these models that combines the targeted usage of existing performance analysis tools, careful selection of new and existing metrics and methodologies to analyze the results, and utilization of domain specific characteristics of DNN training. We also build a new set of tools for memory profiling in all three major frameworks; much needed tools that can finally shed some light on precisely how much memory is consumed by different data structures (weights, activations, gradients, workspace) in DNN training. By using our tools and methodologies, we make several important observations and recommendations on where the future research and optimization of DNN training should be focused.

==> sections/benchmark.tex <==
%\section{Benchmarks} \label{sec:benchmark}

\begin{figure*} [h!]
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/training_seq2seq.pdf}
        \caption{Training seq2seq model}
        \label{fig:training_seq2seq}
    \end{subfigure}%
    \hspace{0.1cm}
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/training_a3c.pdf}
        \caption{Training one a3c agent}
        \label{fig:training_a3c}
    \end{subfigure}
    \caption{The model accuracy during the training for different models.}
    \label{fig:training}
\end{figure*}


%\subsection{Image Classification}
%
%The image classification problem is the most classical deep learning application, as it witnessed the first successful deep neural network (AlexNet~\cite{krizhevsky2012imagenet}) that beats all traditional methods in imagenet challenge 2012. The basic structure of AlexNet is a stack of convolutional and pooling layers, followed by a three connected layers (if the output layer counts). This structure is adopted by subsequent successful CNN models (VGG~\cite{simonyan2014very}, GoogleNet~\cite{szegedy2015going}, ResNet~\cite{he2016deep}) with deeper convolutional stacks.
%
%In this paper we use Inception-v3~\cite{szegedy2016rethinking} and Resnet~\cite{he2016deep} for our image classification benchmark models because of their contributions and current popularity. These two models proposed novel algorithm techniques to allow the network becoming extremely deep.
%
%\subsection{Machine Translation}
%
%Unlike image classification, machine translation, which involves analysis of sequential data, has been using RNNs as its core algorithm. \textit{NMT}\cite{wu2016google} and \textit{Sockeye}\cite{hieber2017sockeye}, which are developed respectively by \textit{TensorFlow} and \textit{Amazon Web Service} team, are selected to be the representative in this area, and \textit{NMT} also claimed that they could achieve comparable results with the Google-Neural-Machine-Translation (GNMT) \cite{wu2016google} system.
%
%The transformer model, recently introduced in \cite{vaswani2017attention}, achieves a new state of the art in translation quality. Unlike RNN based models, it is auto-regressive and uses attention layers as an alternative to recurrence. Since it is maintained by the authors of \cite{vaswani2017attention}, the tensor2tensor implementation, written in Tensorflow, is selected to be the representative for this model.
%
%\subsection{Object Detection}
%
%Object detection is another popular deep learning application related to image processing. This task requires output of the object locations as well as the classification results, and one image generally has multiple objects that need to be reported. A high-level solution to this problem is to use a mechanism to propose region of interests so that an object detection problem is reduces to multiple image classification problems.
%
%Faster-RCNN~\cite{ren2015faster} (published in 2016), which delivers the state-of-the-art results on Pascal VOC datasets, is credited for its high detection accuracy and algorithm design insights. The model is an improvement over the Fast-RCNN~\cite{girshick2015fast} model. It uses a region proposal network to replace the previous inefficient selective search to propose regions for the classification network. A training iteration contains the forward and backward passes of two networks, weight sharing and local fine-tuning. The convolution stack in the Faster R-CNN network (called the \emph{kernel network}) is usually copied from an image classification network such as VGG or ResNet, and its weights are initialized with a fully-trained image classification network. In this work we use a 101-layer ResNet as the \emph{kernel network} for analysis.
%
%Recently YOLO9000~\cite{redmon2016yolo9000} was proposed for the real-time object detection task, achieving faster inference speed than faster-RCNN, and competitive detection accuracy. For now YOLO is still a bit behind in terms of accuracy, we plan to add it when its implementations on the frameworks (TensorFlow, MXNet, CNTK) becomes more mature.
%
%\subsection{Generative Adversarial Networks}
%
%The idea of generative adversarial networks (GAN) was pioneered in 2014~\cite{goodfellow2014generative}, which then revoked great attentions to the unsupervised deep learning area. The basic idea of GAN is to train a generative network and a discriminative network dually. The generator generates data samples that mimic the real samples. The generated samples is then mixed with real samples to form mini-batches, which are then fed to the discriminator that distinguishes generated samples from real samples. The learning goal of the generator is to "fool" the discriminator with output samples that look very real.
%
%The original GAN is known hard to training due to training instability. DCGAN~\cite{radford2015unsupervised} tries to overcome the difficulties with some patches (such as the batch normalization) applied to the original GAN, achieving effective generation results on the LSUN dataset, imagenet-1k and a human-face dataset. The Wasserstein GAN~\cite{arjovsky2017wasserstein} finds the mathematical reasons behind the original GAN which causes the training instability, and solves this issue by applying some extremely succinct modifications to the original GAN. These modifications are theoretically justified and greatly reduce the training instability, which makes Wasserstein GAN the most important milestone of the GAN sub-area. Due its fundamental impact, we choose Wasserstein GAN as our benchmark model despite that its implementation is only available on Tensorflow yet.
%
%\subsection{Speech Recognition}
%
%Deep Speech 2~\cite{amodei2016deep} is an end-to-end speech recognition model from Baidu Research. It is able to recognize both English and Mandarin Chinese, two very distant languages, with a unified model architecture. The model is improved from the previous Deep Speech model in terms of three aspects: the model architecture, big training datasets, and computation scalability. It achieves 7x improvement in training performance comparing to its previous version, showing great potential for deployable production in industry. The Deep Speech 2 model contains two convolutional layers, plus seven regular recurrent layers or Gate Recurrent Units (GRUs), different from the seq2seq model that uses LSTM layers. We use LibriSpeech~\cite{panayotov2015librispeech} as the training dataset due to its availability. This dataset is an automatic speech recognition corpus of approximately 1000 hours of English speech. Due to the large variation between the lengths of the audio data samples, unlike other models that use number of data samples processed per second as the training throughput metric, we use the total duration of audio files processed per second instead.
%
%\subsection{Deep Reinforcement Learning}
%
%The recent developments of RL algorithms have created the first artificial agents to achieve human-level performance across many challenging domains
%%%directly by interacting with their simulated environments. The A3C algorithm~\cite{mnih2016asynchronous}, developed for both single and distributed machine settings, has become one of the most popular DRL techniques in recent times, surpassing DQN training algorithms~\cite{mnih2015human}. A3C relies on asynchronously updated policy and value function networks trained in parallel over several processing threads.


==> sections/implementation.tex <==
\section{Implementation}

Describe the implementation issues for each model on the platforms we choose.
\begin{itemize}
\item Some implementations exist only on one or two platforms.
\item The multi-GPU and multi-machine implementations are sometimes missing, especially multi-machine implementation.
\end{itemize}

==> sections/memory_profiling.tex <==
\section{Memory Usage Analysis}

Discuss per-application memory usage breakdown, analyze the memory usage savings in a distributed environment based on the data functionalities.


==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motiv}

The successes of deep learning algorithms since 2012~\cite{krizhevsky2012imagenet}
have attracted a lot of attention from the system
community and the architecture community. We categorize all existing DNN optimization papers from top system conferences (SOSP, OSDI, NSDI) and architecture conferences (MICRO, ISCA, HPCA, ASPLOS) since 2014 according to the following aspects:

\begin{itemize}
\item \textbf{Training vs. Inference}.
This is determined by
whether the proposed design can be applied to inference, training or both.

\item \textbf{Image-classification-only vs. Other applications}.
We check what applications the corresponding paper uses in its evaluation, are
if there only image classification applications, it is classified as \emph{Image-classification-only}
\begin{comment}
\item
\textbf{System vs. Architecture}. We check whether the proposed optimization
techniques are implemented at the system level (programming language,
OS, library, or networking stack) or architecture level (hardware-based acceleration with
GPUs, FPGAs, ASICs, in-memory computing etc.). Papers that
propose both optimization techniques implemented on hardware and programming
interfaces within a compiler, are considered architectural.
\end{comment}
\end{itemize}

Table~\ref{Related_work_summary} shows our summary results for major systems and
computer architecture conferences. There are more papers which (1) optimize inference over training (23 vs. 15); (2) use image classification
as the \emph{only} application for evaluation (27 vs. 11). We describe our observations and motivations in all the three aspects.

\begin{table*}
    \centering
    \caption{A summary of recent system or architecture papers that focus on improving DNN}
    \label{Related_work_summary}
    \begin{tabular}{|c|c|c|}
        \hline
         & Image Classification Only & Else \\
        \hline
        Training & \cite{alwani2016fused}\cite{chilimbi2014project}\cite{de2017understanding}\cite{ding2017c}\cite{hsieh2017gaia}\cite{judd2016stripes}\cite{kim2016neurocube}\cite{rhu2016vdnn}\cite{song2017pipelayer} &
        \cite{abadi2016tensorflow}\cite{bojnordi2016memristive}\cite{li2014scaling}\cite{pei2017deepxplore}\cite{venkataramani2017scaledeep}\cite{xiao2017tux2} \\ \hline

        Inference & \cite{albericio2017bit}\cite{albericio2016cnvlutin}\cite{chen2016eyeriss}\cite{chi2016prime}\cite{ding2017c}\cite{du2015shidiannao}\cite{gao2017tetris}\cite{judd2016stripes}\cite{likamwa2016redeye}\cite{lu2017flexflow}\cite{parashar2017scnn}\cite{ren2017sc}\cite{shafiee2016isaac}\cite{sharma2016high}\cite{shen2016maximizing}\cite{song2017pipelayer}\cite{yu2017scalpel}\cite{zhang2016cambricon}
        & \cite{abadi2016tensorflow}\cite{du2015neuromorphic}\cite{han2016eie}\cite{ji2016neutrams}\cite{jouppi2017datacenter} \\
        \hline
    \end{tabular}
\end{table*}

%(\emph{TODO: papers that need to be categorized})

%(\emph{DjiNN and Tonic: DNN as a Service and Its Implications for Future Warehouse Scale Computers})

%(\emph{Cambricon: An Instruction Set Architecture for Neural Networks})

%(\emph{Neural Acceleration for GPU Throughput Processors})

%(\emph{Neuromorphic Accelerators: A Comparison Between Neuroscience and Machine-Learning Approaches})

\textbf{Why Study Training Separately from Inference?}
As we previously described, the algorithmic differences between training and
inference create different requirements for the underlying systems and
architecture (both in terms of compute resources, memory, and network and
communication speeds).
%For example, due to
%the backward pass and weight update, the training procedure needs to withhold a
%large amount of intermediate results in memory. This demands the memory
%capacity of a modern DNN accelerator in order of gigabytes. The training also
%needs to intensively process a large amount of data to avoid overfitting,
%throughput is then a major performance metric. On the other hand, the inference
%procedure is much more light weighted. It process a data sample in only one
%forward pass, the latency of processing a data sample becomes more important
%than throughput. The memory footprint is only in order of metabytes since no
%intermediate result needs to stay in memory. The major consumer of the memory
%becomes the weights of the model, which leads to very different approaches in
%terms of reducing memory footprint from the training case.
Optimization techniques that are tailored for inference are usually either difficult
to port directly (e.g., ~\cite{rastegari2016xnor}) or not applicable at all for training~\cite{han2015deep,han2016eie,wu2016quantized}.
Many optimizations designed for training (e.g., parallelized stochastic gradient descent~\cite{zinkevich2010parallelized,recht2011hogwild}, dataflow representation~\cite{abadi2016tensorflow,chen2015mxnet,bergstra2010theano}, asynchronous communication~\cite{li2014scaling}) does not make a lot of sense
for inference as they target bottlenecks that are either less important or not important
at all for inference.


\textbf{A Case for a More Diverse Benchmark Pool}
Deep learning has achieved the state-of-the-art results in many application domains
such as object detection~\cite{ren2015faster,redmon2016yolo9000}, machine translation~\cite{sutskever2014sequence,vaswani2017attention}, speech recognition~\cite{amodei2016deep,DBLP:journals/corr/abs-1708-06073},
but image classification is still the most popular application used to evaluate different
designs, and CNNs remain the most widely-used model for system and hardware researchers.
As a result, a large variety of modern DNN models does not receive proper attention and
deep analysis. The major problem is that the key bottlenecks of image classification
models could be (and, in fact, are) very different from these other models as we
show later in this paper.
Prior works~\cite{adolf2016fathom} somewhat addressed this diversity issue by introducing
benchmarks from applications like speech recognition and reinforcement
learning. But unfortunately new DNN models and algorithms evolve at a rapid pace, making
the models used in these prior works almost completely outdated.

We believe that a proper open-sourced DNN training benchmark suite is a must, and
it should have enough breadth to cover major important application areas with
the state-of-the-art models to reflect the workload of current
and future DNNs in these areas. In this work, we propose such a benchmark suite
that covers \emph{six} application areas and \emph{eight} state-of-the-art models.



\textbf{A Need for Holistic Analysis}
Some existing optimization techniques designed specifically for training
(asynchronous communication~\cite{li2014scaling}, dataflow
representation~\cite{abadi2016tensorflow,bergstra2010theano,chen2015mxnet}) are
based on either some empirical evidence or simple intuition on where the major
bottlenecks could be.
These techniques proved to be efficient in improving DNN training performance, but to see
further optimization opportunities in training, there is a need for
a more comprehensive study that would apply a more holistic analysis across all major
potential bottlenecks (both at systems and architecture levels)
and would provide some potential hints to the ML developers on how their
current models can be improved. In our work, we present a new set of methodologies
for this holistic analysis (described in Section~\ref{sec:method}) and then apply
this analysis to our new benchmark pool (see Section~\ref{sec:performance}). Our analysis
reveals several interesting observations and suggestions to improve performance
of these benchmarks that we summarize in Section~\ref{sec:summary}.



\begin{comment}
%TODO: Our analysis reveals how computation resources are utilized. This can be included in section 4

%TODO: this should be a part of methodology!

\subsection{Why do We Analyze on the System Level?}

Deep learning researchers need certain flexibility to go through the training process over and over to find out the best hyper-parameter configurations. Even more programming liberty is often required to define a new type of layer, fine-tuning a subset of weights, or manipulating hyper-parameters during training. The desired programmability is provided by the system level framework rather than architecture. A DNN framework can make DNN programming much more convenient, it would also increase the complexity of the overall abstractions from user programs to hardware. The performance bottlenecks could then come from different sources. Such a bottleneck could be:

\begin{itemize} \item \textbf{Computation.} For most of the networks for image
classification, the training is heavily computation-intensive, therefore
bounded by computation. We will backup this claim in section
\ref{sec:performance}.  \item \textbf{Memory.} We will show that in
\ref{sec:performance}, for recurrent neural networks the training performance
is greatly affected by mini-batch size, and the mini-batch. Increasing the
mini-batch size can significantly improve the training performance, however
this size is limited by physical memory capacity of a single GPU.  \item
\textbf{Interconnect and communication bandwidth.} To train a DNN in a
distributed environment will introduce the need for communications among CPUs
and GPUs. The communication costs may affect the training performance as well.
We will analyze in detail in section \emph{TODO: ref of later section}.
\end{itemize}

Identifying whether the training performance is bounded by computation, memory
or communication is not easy. Existing profiling tools (e.g. vTune, nvprof,
etc.) have no domain knowledge about the algorithm logic, and can only capture
information within their own scopes. Therefore to do a holistic analysis, the
profiling results generated by these tools need to be correctly interpreted
with domain knowledge, and partial information also needs to be put together to
make claims about the bottlenecks. In this paper, we develop a tool chain to do
such holistic analysis. We believe such a study can provide insights for both
system and architecture researchers.

\end{comment}

